Computing zeta functions of algebraic curves using Harvey's trace formula

We present a new method for computing the zeta function of an algebraic curve over a finite field. The algorithm relies on a trace formula of Harvey to count points on a plane model of the curve. The zeta function of the curve is then obtained by making corrections at singular points. We report on an implementation and provide some examples in MAGMA which demonstrate an improvement over Tuitman's algorithm.

==> bib.bbl.tex <==
\providecommand{\bysame}{\leavevmode\hbox to3em{\hrulefill}\thinspace}
\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
}
\providecommand{\href}[2]{#2}
\begin{thebibliography}{vzGG03}

\bibitem[AH01]{AH-counting}
Leonard~M. Adleman and Ming-Deh Huang, \emph{Counting points on curves and
  abelian varieties over finite fields}, J. Symbolic Comput. \textbf{32}
  (2001), no.~3, 171--189. \MR{1851164 (2002j:14027)}

\bibitem[AKR10]{AKR-picard}
Timothy~G. Abbott, Kiran~S. Kedlaya, and David Roe, \emph{Bounding {P}icard
  numbers of surfaces using {$p$}-adic cohomology}, Arithmetics, geometry, and
  coding theory ({AGCT} 2005), S\'emin. Congr., vol.~21, Soc. Math. France,
  Paris, 2010, pp.~125--159. \MR{2856564}

\bibitem[Ber08]{Ber-fastmult}
Daniel~J. Bernstein, \emph{Fast multiplication and its applications},
  Algorithmic number theory: lattices, number fields, curves and cryptography,
  Math. Sci. Res. Inst. Publ., vol.~44, Cambridge Univ. Press, Cambridge, 2008,
  pp.~325--384. \MR{MR2467550 (2010a:68186)}

\bibitem[BGS07]{BGS-recurrences}
Alin Bostan, Pierrick Gaudry, and {\'E}ric Schost, \emph{Linear recurrences
  with polynomial coefficients and application to integer factorization and
  {C}artier-{M}anin operator}, SIAM J. Comput. \textbf{36} (2007), no.~6,
  1777--1806. \MR{2299425 (2008a:11156)}

\bibitem[Bom78]{Bom-exponential}
E.~Bombieri, \emph{On exponential sums in finite fields. {II}}, Invent. Math.
  \textbf{47} (1978), no.~1, 29--39. \MR{0506272 (58 \#22072)}

\bibitem[CDV06]{CDV-nondegenerate}
W.~Castryck, J.~Denef, and F.~Vercauteren, \emph{Computing zeta functions of
  nondegenerate curves}, IMRP Int. Math. Res. Pap. (2006), Art. ID 72017, 57.
  \MR{2268492 (2007h:14026)}

\bibitem[CGH14]{CGH-wilson}
Edgar Costa, Robert Gerbicz, and David Harvey, \emph{A search for {W}ilson
  primes}, Math. Comp. \textbf{83} (2014), no.~290, 3071--3091. \MR{3246824}

\bibitem[CV09]{CV-nondegeneracy}
Wouter Castryck and John Voight, \emph{On nondegeneracy of curves}, Algebra
  Number Theory \textbf{3} (2009), no.~3, 255--281. \MR{2525551 (2010g:14033)}

\bibitem[Ger07]{Ger-relative}
Ralf Gerkmann, \emph{Relative rigid cohomology and deformation of
  hypersurfaces}, Int. Math. Res. Pap. IMRP (2007), no.~1, Art. ID rpm003, 67.
  \MR{MR2334009 (2008f:14036)}

\bibitem[Har07]{Har-kedlaya}
David Harvey, \emph{Kedlaya's algorithm in larger characteristic}, Int. Math.
  Res. Not. IMRN (2007), no.~22, Art. ID rnm095, 29. \MR{2376210 (2009d:11096)}

\bibitem[Har14]{Har-avgpoly}
\bysame, \emph{Counting points on hyperelliptic curves in average polynomial
  time}, Ann. of Math. (2) \textbf{179} (2014), no.~2, 783--803.

\bibitem[HS14a]{HS-hassewitt}
David Harvey and Andrew~V. Sutherland, \emph{Computing {H}asse-{W}itt matrices
  of hyperelliptic curves in average polynomial time}, LMS J. Comput. Math.
  \textbf{17} (2014), no.~suppl. A, 257--273. \MR{3240808}

\bibitem[HS14b]{HS-hassewitt2}
\bysame, \emph{Computing {H}asse-{W}itt matrices of hyperelliptic curves in
  average polynomial time, {II}}, to appear in {\it Frobenius Distributions},
  Contemporary Mathematics, AMS; preprint at
  \url{http://arxiv.org/abs/1410.5222}, 2014.

\bibitem[Hub10]{Hub-unramified}
Hendrik Hubrechts, \emph{Fast arithmetic in unramified {$p$}-adic fields},
  Finite Fields Appl. \textbf{16} (2010), no.~3, 155--162. \MR{2610706
  (2011d:11277)}

\bibitem[Ked01]{Ked-hyperelliptic}
Kiran~S. Kedlaya, \emph{Counting points on hyperelliptic curves using
  {M}onsky-{W}ashnitzer cohomology}, J. Ramanujan Math. Soc. \textbf{16}
  (2001), no.~4, 323--338. \MR{MR1877805 (2002m:14019)}

\bibitem[Lau04]{Lau-manyvar}
Alan G.~B. Lauder, \emph{Counting solutions to equations in many variables over
  finite fields}, Found. Comput. Math. \textbf{4} (2004), no.~3, 221--267.
  \MR{MR2078663 (2005f:14048)}

\bibitem[Lau06]{Lau-recursive}
\bysame, \emph{A recursive method for computing zeta functions of varieties},
  LMS J. Comput. Math. \textbf{9} (2006), 222--269. \MR{2261044 (2007g:14022)}

\bibitem[LW08]{LW-counting}
Alan G.~B. Lauder and Daqing Wan, \emph{Counting points on varieties over
  finite fields of small characteristic}, Algorithmic number theory: lattices,
  number fields, curves and cryptography, Math. Sci. Res. Inst. Publ., vol.~44,
  Cambridge Univ. Press, Cambridge, 2008, pp.~579--612. \MR{2467558
  (2009j:14029)}

\bibitem[Min10]{Min-superelliptic}
Moritz Minzlaff, \emph{Computing zeta functions of superelliptic curves in
  larger characteristic}, Math. Comput. Sci. \textbf{3} (2010), no.~2,
  209--224. \MR{2608297}

\bibitem[Pap94]{Pap-complexity}
Christos~H. Papadimitriou, \emph{Computational complexity}, Addison-Wesley
  Publishing Company, Reading, MA, 1994. \MR{1251285 (95f:68082)}

\bibitem[Pil90]{Pil-abelian}
J.~Pila, \emph{Frobenius maps of abelian varieties and finding roots of unity
  in finite fields}, Math. Comp. \textbf{55} (1990), no.~192, 745--763.
  \MR{1035941 (91a:11071)}

\bibitem[PT13]{PT-deformation}
Sebastian Pancratz and Jan Tuitman, \emph{Improvements to the deformation
  method for counting points on smooth projective hypersurfaces}, to appear in
  Foundations of Computational Mathematics, posted electronically 6th January
  2015, 2013.

\bibitem[Sch85]{Sch-elliptic}
Ren{\'e} Schoof, \emph{Elliptic curves over finite fields and the computation
  of square roots mod {$p$}}, Math. Comp. \textbf{44} (1985), no.~170,
  483--494. \MR{777280 (86e:11122)}

\bibitem[Ser65]{Ser-zeta-L}
Jean-Pierre Serre, \emph{Zeta and {$L$} functions}, Arithmetical {A}lgebraic
  {G}eometry ({P}roc. {C}onf. {P}urdue {U}niv., 1963), Harper \& Row, New York,
  1965, reprinted in \cite{Ser-oeuvres2}, pp.~82--92. \MR{0194396 (33 \#2606)}

\bibitem[Ser86]{Ser-oeuvres2}
\bysame, \emph{{\OE}uvres. {V}ol. {II}}, Springer-Verlag, Berlin, 1986,
  1960--1971. \MR{926690 (89h:01109b)}

\bibitem[SV13]{SV-fewnomial}
Steven Sperber and John Voight, \emph{Computing zeta functions of nondegenerate
  hypersurfaces with few monomials}, LMS J. Comput. Math. \textbf{16} (2013),
  9--44. \MR{3033943}

\bibitem[Tui14a]{Tui-general}
Jan Tuitman, \emph{Counting points on curves: the general case}, preprint at
  \url{http://arxiv.org/abs/1412.7217}, 2014.

\bibitem[Tui14b]{Tui-P1}
\bysame, \emph{Counting points on curves using a map to {$P^1$}}, to appear in
  Mathematics of Computation, posted electronically 10th July 2015, 2014.

\bibitem[vzGG03]{vzGG-compalg}
Joachim von~zur Gathen and J{\"u}rgen Gerhard, \emph{Modern computer algebra},
  second ed., Cambridge University Press, Cambridge, 2003. \MR{2001757
  (2004g:68202)}

\bibitem[Wan08]{Wan-zeta}
Daqing Wan, \emph{Algorithmic theory of zeta functions over finite fields},
  Algorithmic number theory: lattices, number fields, curves and cryptography,
  Math. Sci. Res. Inst. Publ., vol.~44, Cambridge Univ. Press, Cambridge, 2008,
  pp.~551--578. \MR{2467557 (2010c:11157)}

\end{thebibliography}
